All Politics is Local: Redistricting via Local Fairness

In this paper, we propose to use the concept of local fairness for auditing and ranking redistricting plans. Given a redistricting plan, a deviating group is a population-balanced contiguous region in which a majority of individuals are of the same interest and in the minority of their respective districts; such a set of individuals have a justified complaint with how the redistricting plan was drawn. A redistricting plan with no deviating groups is called locally fair. We show that the problem of auditing a given plan for local fairness is NP-complete. We present an MCMC approach for auditing as well as ranking redistricting plans. We also present a dynamic programming based algorithm for the auditing problem that we use to demonstrate the efficacy of our MCMC approach. Using these tools, we test local fairness on real-world election data, showing that it is indeed possible to find plans that are almost or exactly locally fair. Further, we show that such plans can be generated while sacrificing very little in terms of compactness and existing fairness measures such as competitiveness of the districts or seat shares of the plans.

==> discarded_experiments.tex <==


% \noindent {\bf Speeding up the algorithm.}
%The time complexity of the algorithm is still prohibitively high. In our experiments, we use two approaches to speed it up, and present details in Appendix~\ref{ss:dp_details}. First, we use suitable interpolation to assume $\tau(v) = \rho(v)$. We further relax the constraint on state $A[v, i]$ so that for a subtree $W \subset T_v$, $\rho(W) \leq i$. This ensures that $A[v, i]$ is non-decreasing in $i$ and $B_{v, i}[j, x]$ is non-decreasing in $x$, allowing us to devise pruning strategies to avoid exhaustively examining every case in Equation~\ref{horizontal_dp}. However, this introduces a one sided error, in that the algorithm may find a deviating group that does not have a feasible population size.  We finally round the population of precincts: we introduce a threshold $P$ and scale down each $\rho(v)$ to the largest multiple of $P$ that is at most $\rho(v)$. This limits the total number of population levels the algorithm must consider, and the running time is reduced to $O(\abs{V} \cdot (\frac{\sigma}{P})^3 \cdot \Delta(T))$. 

%we adopt further strategies to bring down the complexity of the algorithm, with a potential sacrifice in the precision of the algorithm. We present these strategies in the $\tau(v) = \rho(v)$ special case.   This ensures that $A[v, i]$ is non-decreasing in $i$ and $B_{v, i}[j, x]$ is non-decreasing in $x$, allowing us to devise pruning strategies to avoid exhaustively examining every case in Equation~\ref{horizontal_dp}. %update the $\max$ in  in constant time.   We present the details in .


%Due to the intractability of the auditing problem, we develop frameworks for generating candidate sets of deviating groups, and audit using this set. In other words, given any feasible redistricting plan $\Pi$, we seek to either determine that $\Pi$ is \emph{not locally fair} by finding one or multiple deviating groups with respect to $\Pi$, or classify $\Pi$ as \emph{likely fair}, in which case $\Pi$ is either indeed locally fair or `close' to being locally fair in that our candidate set contained no deviating groups with respect to $\Pi$. 
% it is significantly harder to find deviating groups for than it is for other unfair maps.
% \todo{expand what we mean by `likely fair'-- just say locally fair (with respect to the ensemble, we expect probability it is not fair to be small).}


%According to the results, we can then either directly output the set of locally fair plans, or rank the plans in $\ens$ by their unfairness score, and output the top ones. This can be seemed as \emph{filtering out} maps which are not locally fair. Therefore, in this section, we focus our discussion on the \audit\ problem. 

%More broadly, given the fixed district ensemble $\Delta$ as a baseline, one can analyze the sets of deviating groups $\Tilde{W}^\ast_{\text{B}}(\Pi)$ and $\Tilde{W}^\ast_{\text{R}}(\Pi)$ found in Algorithm~\ref{alg:audit} in a fine-grained sense. This broadens the usage of Algorithm~\ref{alg:audit} to the task of \emph{determining the best candidate plan} in terms of local fairness in (or obtaining a \emph{ranking} of) a given set of candidate redistricting plans; here, the candidate set can come from any arbitrary sources and may even be identical to the plan ensemble $\ens$ used for audition. That is,  one may  then use $\ens$ itself in Algorithm~\ref{alg:generate} to determine the top (fairest) plans in $\ens$, and output these plans as candidate plans. In Section~\ref{s:results}, we empirically demonstrate this approach using real electoral data to generate fair plans.



%As discussed above, our speedup strategies are designed with the desired one-side error property in mind. In fact, the algorithm itself (in its exact form) also similarly errs on the safe side in terms of compactness requirements: the entire algorithm ignores any possible compactness requirements of a deviating group and only requires that the subtree $W$ is connected. Therefore, if the algorithm does not find any subtree of $T$ with respect to $\Pi$ such that a majority of its voters are unhappy voters of the same color, then we can safely conclude that there is no compact deviating group $W$ that is a subtree of $T$ regardless of what is the compactness concept. On the other hand, as manifested in the experimental results, the ``deviating groups'' (subgraphs satisfying $A'[v,i] > \frac{i}{2}$ and $i \in [(1-\eps)\sigma, (1+\eps)\sigma]$) found by this algorithm may be spurious (since it is not necessarily the case that $A[v,i] > \frac{i}{2}$) or not compact, in which case one can add a verification step to the algorithm to filter out such spurious deviating groups.

%It is known that random spanning trees are deeply tied to the cut set-based compactness objective~\cite{procaccia2022compact}, and the deviating groups for the original \audit\ problem are likely to be preserved by a sufficiently large set of spanning trees (i.e., a deviating group $W$ is a subtree of some tree $T \in \mathcal{T}$). In other words, if no deviating group is found for all spanning trees in $\mathcal{T}$ when $\abs{\mathcal{T}}$ is large enough, $\Pi$ is more likely to be locally fair. However, the reversed direction is not always true: as shown in our experiments, not all candidate deviating groups (as subtrees of spanning trees of $G$) are compact subgraphs of $G$. In other words, there is an implicit relaxation in compactness requirements from optimizing for deviating groups in a general graph to that on a tree.








%it can be used as a \emph{filtering} step before more systematic (but computationally extensive) methods are deployed to further analyze the likely fair plans, whereas the plans deemed unfair in the first step needs no further investigation. 
%Finally, it provides a natural ways for quantifying the degree of unfairness of any redistricting plan $\Pi$: by its enumerative nature, it approximates the unfairness measure $\Tilde{\unf}(\Pi)$ alongside auditing $\Pi$. It is then natural to \emph{rank} the plans in $\ens$ by their $\Tilde{\unf}(\Pi)$ values.

%\paragraph{\audit\ Problem.} 
%For the auditing problem, we first generate an ensemble $\ens$ of $t$ feasible plans by running \recom\ for $t \cdot s$ steps such that each plan $\Pi_j \in \ens$ is the result of a $s$-step \recom\ chain. We then obtain the resulting set of potential deviating groups $\Delta = \{D \subseteq V \mid \exists j \ \text{s.t.} \ D \in \Pi_j \in \ens\}$. Then, to audit the given plan $\Pi$, we check whether each district $D \in \Delta$ is a red or blue deviating group with respect to $\Pi$. Let $\Tilde{W}^\ast_{\text{B}}(\Pi) \coloneqq \bigcup\{D \in \Delta \mid D \text{ is a blue deviating group of $\Pi$}\}$ and $\Tilde{W}^\ast_{\text{R}}(\Pi) \coloneqq \bigcup\{D \in \Delta \mid D \text{ is a red deviating group of $\Pi$}\}$ denote the collections of blue and red deviating groups found in this process; we then approximate and $\unf(\Pi)$ by using $\Tilde{W}^\ast_{\text{B}}(\Pi)$ and $\Tilde{W}^\ast_{\text{R}}(\Pi)$ in place of $W^\ast_{\text{B}}(\Pi)$ and $W^\ast_{\text{R}}(\Pi)$.
%We detail this process in~\ref{alg:audit}, assuming that $\eps$ and $k$ are fixed. 

\iffalse
\IncMargin{2em}
\begin{algorithm}[h]
    \SetKwFunction{gen}{Generate-$\Delta$($t, s$)}
    \SetKwFunction{aud}{Audit($G, \Delta$)}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{$G, c$, feasible redistricting plan $\Pi$}
    \Output{$\Tilde{\unf}(\Pi)$}
    \BlankLine
    $\Delta, \ens \leftarrow$ \gen \\  
    \SetKwProg{myproc}{}{}{}
    \myproc{\aud:}{
    % \aud:\\ 
    $\Tilde{W}^\ast_{\text{B}}(\Pi), \Tilde{W}^\ast_{\text{R}}(\Pi) \leftarrow \varnothing$ \\
    \For{$D$ in $\Delta$}{
        \If{$D$ is a blue $c$-deviating group in $G$ w.r.t $\Pi$}{
            $\Tilde{W}^\ast_{\text{B}}(\Pi) \leftarrow \Tilde{W}^\ast_{\text{B}}(\Pi) \cup \{D\}$ }
        \If{$D$ is a $c$-red deviating group in $G$ w.r.t $\Pi$}{
            $\Tilde{W}^\ast_{\text{R}}(\Pi) \leftarrow \Tilde{W}^\ast_{\text{R}}(\Pi) \cup \{D\}$ }
    }
    $\Tilde{\unf}(\Pi) \leftarrow \frac{\beta(\Tilde{W}^\ast_{\text{B}}(\Pi)) \cdot \tau(\Tilde{W}^\ast_{\text{B}}(\Pi)) + \gamma(\Tilde{W}^\ast_{\text{R}}(\Pi)) \cdot \tau(\Tilde{W}^\ast_{\text{R}}(\Pi))}{\tau(V)}$\\
    \Return{$\Tilde{\unf}(\Pi)$}}
    \BlankLine
    \SetKwProg{myproc}{}{}{}
    \myproc{\gen:}{
        $\Delta, \ens \leftarrow \varnothing, \varnothing$ \\
        \For{$i \in 1, \dots, t$}{
            $\Pi \leftarrow \recom$ districting after $s$ steps  \\
            $\Delta \leftarrow \Delta \cup \Pi$ \\
            $\ens \leftarrow \ens \cup \Pi$
        }
        \Return{$\Delta, \ens$}} 
    \caption{Auditing Algorithm}
    \label{alg:audit}
\end{algorithm}
\fi

% \paragraph{\generation\ Problem.} 
% For the map generation problem, we now also generate a set of candidate fair maps, and use our auditing algorithm to filter out the plans which are not locally fair. We use the ensemble generated by \recom\ as the set of potential fair maps. See Algorithm~\ref{alg:generate} for details. 

% \IncMargin{2em}
% \begin{algorithm}
%     \SetKwFunction{gen}{Generate-$\Delta$($t, s$)}
%     \SetKwFunction{aud}{Audit($\Pi, \Delta$)}
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \Input{$G, \rho, \tau, \gamma, \beta, \eps, c, k$}
%     \Output{$\mathcal{F}$ set of locally fair maps}
%     \BlankLine
%     $\Delta, \ens \leftarrow$ \gen \\ 
%     $\mathcal{F} \leftarrow \varnothing$  \\ 
%     \For{Plan $\Pi \in \ens$}{
%         $\Tilde{\tvdg}(\Pi), \Tilde{\unf}(\Pi) \leftarrow$ \aud  \\ 
%         \If{$\Tilde{\tvdg}(\Pi) = \Tilde{\unf}(\Pi) = 0$}{
%             $\mathcal{F} \leftarrow \mathcal{F} \cup \{\Pi\}$ \\ 
%         }
%     }
%     \Return{$\mathcal{F}$}
%     \caption{Generation Algorithm}
%     \label{alg:generate}
% \end{algorithm}





%%%%%%%%%%%%%%%%
Interpolated Voter Labels

% To check whether maps are locally fair, we require knowing the total number of voters, $\tau$, and the red and blue ratio, $\gamma, \beta$. 
% In our experimental setup (see Section~\ref{ss:set-up}), we generated these labels based on the results from one election. 
% %Specifically, if $r_v, b_v$ are the number of red and blue voters, we set $\gamma_v = r_v/(r_v+b_v)$ and $\beta_v = b_v/(r_v+b_v)$ for each precinct $v$. 
% The obvious downside to this approach is that different sets of voters show up to different elections, and the ratio of red and blue votes fluctuate between elections. 
% Additionally, the total number of voters differs from the total population. 

%We discuss results using this method below. Another possible method is to do this interpolation in the district-level, so that the rate of red/blue non-voters is modeled by the rate of aggregated red/blue votes in each district. We note that there is no single correct method to assign voter labels.


%To assign labels to portions of the population who did not vote, one possible way is to 
% We now repeat the experiments in Sections~\ref{ss:achievability} and~\ref{ss:compatibility} with interpolated voter label data. Recall that for each precinct $v$, we collect the number of total votes for the Republican party $r_v$ and the total vote amount for the Democrat party $b_v$ in the 2016 presidential election from~\cite{mgggstates}. For the interpolated voter labels, we keep $\gamma(v) = r_v/(r_v+b_v)$ and $\beta(v) = 1-r_v$ as the relative portion of red (resp. blue) votes in the precinct $v$, but set $\tau(v) = \rho(v)$ instead. This is equivalent to assuming every individual in precinct $v$ votes, and the rate of blue- and red-favoring individual is proportional to the actual votes in the election.

% \paragraph{Number of locally fair maps.}
% \begin{table}[!htbp]
%     \centering
%     \begin{tabular}{||c c c c||} 
%     \hline
%     State & $c = 0.5$ & $c = 0.55$ & $c = 0.6$ \\ \hline \hline
%     NC & 5.2\%  & 61.1\% & 81.6\% \\ \hline
%     TX & 49.1\% & 68.5\% & 83.4\% \\ \hline
%     PA & 38.8\% & 99.2\% & 99.5\% \\ \hline
%     WI & 99.7\% & 99.8\% & 100.0\% \\ \hline
%     \end{tabular}
%     \caption{Percentages of plans without $c$-deviating groups}
%     \label{tab:achievability_interpolated}
% \end{table}

% Table~\ref{tab:achievability_interpolated} summarizes the percentages of plans in $\ens_\text{X}$ without $c$-deviating groups in $\Delta_\text{X}$ for $c \in \{0.5, 0.55, 0.6\}$. In general, more plans are identified as locally fair using the interpolated voter label data compared to the default setting. Figure~\ref{fig:compatibility_interpolated} repeats the experiments in Section~\ref{ss:compatibility} using interpolated voter labels; as most of the WI plans are identified locally fair, we omit the WI results in Figure~\ref{fig:compatibility_interpolated}. Although there are less deviating groups across all plans, results using interpolated voter label data still show that the seat share outcomes and the average partisanship in fair plans are comparable to that in the overall ensemble.


% \begin{figure}[!htbp]
% \centering
%     \begin{subfigure}[b]{\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/box_plots/seat_nctxpa_interp.png}
%     \caption{Seat share outcomes (Minor\%) among subsets of plans.}
%     \label{fig:seat_distribution_interpolated}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{\textwidth}
%     \centering
% %     \includegraphics[width=\textwidth]{fig/box_plots/part_nctxpa_interp.png}
% %     \caption{Average partisanship among subsets of plans.}
% %     \label{fig:partisanship_interpolated}
% %     \end{subfigure}

% \caption{Distribution of fairness metrics among generated plans}
% \label{fig:compatibility_interpolated}
% \end{figure}

 Note that the total population of a precinct is not equal to the number of eligible voters, so this is an overestimation of the number of possible voters.
Another advantage of this approach is that the dynamic programming algorithm becomes more efficient.




% \subsection{Consistency Between Auditing Approaches}
% \label{ss:dp_vs_ensemble}



\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\textwidth]{fig/DP/strength_dev_groups.png}
    \caption{Box plots of strengths of deviating groups found by DP}
    \label{fig:strength_dg}
\end{figure}

In order to systematically substantiate the difference between auditing fair and unfair plans, we run our dynamic program on $\abs{\mathcal{T}} = 5$ random spanning trees of $G$ with rounding parameter $P = 750$ on the the three subsets of plans for NC: the top $2\%$ ``fairest'' plans $\ens^\ast$ (identified as fair via the ensemble based auditing method using both 2012 and 2016 voter labels), the bottom $1\%$ fairest plans (ranked by $\unf$), and a set of $1\%$ plans ranked around the 50th percentile among all plans (ranked by $\unf$).  For each deviating group found in this process, we measure its strength and the Polsby-Popper scores. Figure~\ref{fig:strength_dg} plots the distribution of strengths of compact (Polsby-Popper score $\geq .14$) deviating groups found by the DP for the three subsets of plans. These results show that the strengths of deviating groups for fair plans (according to ensemble based auditing) are considerably lower than that for average or unfair plans. 

\todo{Current data uses 20 tree for the fairest plans. We may run more and make every set 20 trees.}

% \subsection{Alternative Unfairness Measures}
% \label{ss:tvdg}
% Throughout our results, we use the unfairness score $\unf(\Pi)$ to rank the unfairness of redistricting plans. One alternative method is to compute the total percentage of voters that appear in deviating groups:

% \begin{definition}[Voters in deviating groups]
% For a feasible redistricting plan $\Pi$ of $G$, its \emph{total voter percentage in deviating groups} is given by
% \[ \tnf(\Pi) \coloneqq \frac{\tau(W^\ast_{\text{B}}(\Pi) \cup W^\ast_{\text{R}}(\Pi))}{\tau(V)}. \]
% \end{definition}

% It is straightforward to extend Algorithm~\ref{alg:audit} to compute approximate values of $\tnf$. We then repeat the experiments in Section~\ref{ss:robustness} using $\tnf$ instead of $\unf$ as the ranking metric. The results are shown in Figure~\ref{fig:robustness_tvdg}. Results show that the concept of local fairness remains robust between using voter labels from different elections when the alternative metric $\tnf$ is used in place of $\unf$.

% \begin{figure}[!htbp]
% \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/tvdg_12.png}
%     \caption{\tnf$(\Pi)$ w.r.t. 2012 election}
%     \label{fig:unhp_pop_dg_12}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/tvdg_16.png}
%     \caption{\tnf$(\Pi)$ w.r.t. 2016 election}
%     \label{fig:unhp_pop_dg_16}
%     \end{subfigure}
    
% \caption{Histograms of \tnf$(\Pi)$ cross-compared between 2012 and 2016 North Carolina elections.}
% \label{fig:robustness_tvdg}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/districtings/map_4_dev_group_111_13.png}
%     % \caption{population in deviating groups, 2012}
%     \label{fig:map4-dg2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/districtings/map_4_dev_group_224_8.png}
%     % \caption{unhappy population in deviating groups, 2012}
%     \label{fig:map4-dg2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/districtings/map_4_dev_group_869_10.png}
%     \label{fig:map4-dg3}
%     \end{subfigure}
% \caption{Three deviating groups of a plan, each with the same set of unhappy precincts.}
% \label{fig:core_uhp_precincts}
% \end{figure}

% However, we choose $\unf$ as the primary unfairness metric because it better captures the ``core-peripheral'' phenomenon in deviating groups. We find that it is common for the same set of ``core'' precincts (that are unhappy and of the same color) to form multiple different deviating groups by ``pulling in'' different sets of ``peripheral'' neighboring precincts that are not essential to the deviating nature of the formed district. Figure~\ref{fig:core_uhp_precincts} visualize an example of three distinct deviating groups for NC with identical set of unhappy precincts. Ideally, we treat these deviating groups as a single one; had this been a real case, the group of voters that initializes their justified complaint would be exactly the same. By definition, this is correctly reflected in $\unf$ but not $\tnf$, as the latter counts all three ``peripheral'' sets toward the metric.

==> hardness.tex <==
\section{Hardness of Auditing and Generation} 
\label{ss:hardness}

\begin{theorem} \label{thm:audit_hardness}
\audit\ is \textsf{NP}-complete.
\end{theorem}

\begin{proof}
We reduce the \textsf{NP}-complete Connected $k$-Subgraph Problem on Planar Graphs with Binary Weights (\ckspb)~\cite{hochbaum1994node} to the \audit\ problem. 
Given a connected planar graph $\mathsf{G} = (\mathsf{V}, \mathsf{E})$ where $\mathsf{V} = \{\mathsf{v}_1, \mathsf{v}_2, \ldots, \mathsf{v}_{\abs{\mathsf{V}}}\}$, a vertex weight $\omega(\mathsf{v}_i) \in \{0,1\}$ for each $\mathsf{v}_i \in \mathsf{V}$, a size $M \geq 2$, and a targeted total weight $\Omega \in \mathbb{Z}^{+}$,\footnote{We use $M$ and $\Omega$ here to avoid confusing with the notations $k$ and $W$ in our problem.} the decision version of \ckspb\ asks whether there is a subset $\mathsf{W} \subseteq \mathsf{V}$ of $M$ vertices such that its induced subgraph $\mathsf{H} \subseteq \mathsf{G}$ is connected and $\sum_{\mathsf{v}_i \in \mathsf{W}} \omega(\mathsf{v}_i) \geq \Omega$. Here it is assumed that $M \leq \abs{\mathsf{V}}$ and $\omega(\mathsf{v}_i) < \Omega$ for each $\mathsf{v}_i \in \mathsf{V}$; otherwise the problem is trivial. 

Given an arbitrary instance of \ckspb, we construct an instance for \audit\ as follows. For each vertex $\mathsf{v}_i \in \mathsf{V}$, we construct two precinct nodes $v_i$ and $u_i$, and an edge between $v_i$ and $u_i$. For each edge $(\mathsf{v}_i, \mathsf{v}_j) \in \mathsf{E}$, we construct an edge between $v_i$ and $v_j$. Hence, the resulting graph $G = (V,E)$ has $2\abs{\mathsf{V}}$ precinct nodes and $\Paren{\abs{\mathsf{V}}+\abs{\mathsf{E}}}$ edges, and is still planar. 

For all $i = 1, 2, \ldots, \abs{\mathsf{V}}$, we let $\rho(v_i) = \tau(v_i) = 2M \Omega$ and $\gamma(v_i) = \Paren{\frac{M-1}{2M}+\frac{\omega(\mathsf{v}_i)}{2\Omega}}$; note that each $\gamma(v_i)$ is in $(0, 1)$ and each $\gamma(v_i) \cdot \tau(v_i)$ is an integer. For all $i$, we let $\rho(u_i) = \tau(u_i) = 2M(M-1)\Omega$, and $\gamma(u_i) = 0$. We call the precinct nodes $v_i$ \textit{regular} and the precinct nodes $u_i$ \textit{auxiliary}. Let $k = \abs{\mathsf{V}}$, $c = 1/2$, and pick $\eps$ such that $0 < \eps < \frac{1}{M}$. Finally, let $\Pi = \{D_1, D_2, \ldots, D_k\}$, where $D_i = \{ v_i, u_i \}$ for all $i = 1, 2, \ldots, k$. Observe that we have $\beta(D_i) > \frac{1}{2}$ for all $i = 1, 2, \ldots, k$, i.e., we have $B_\Pi = V$ and $R_\Pi = \varnothing$. Note that since $0 < \eps < \frac{1}{M}$, we have $(2M^2 - 2M) \Omega < (1-\eps)2M^2 \Omega$ and $(2M^2 + 2M) \Omega > (1+\eps)2M^2 \Omega$, and thus every feasible district has total population exactly $2M^2 \Omega$.

Suppose the \ckspb\ instance is a $\texttt{Yes}$ instance, i.e., there is a subset $\mathsf{W} \subseteq \mathsf{V}$ of $M$ vertices such that its induced subgraph $\mathsf{H} \subseteq \mathsf{G}$ is connected, and $\sum_{\mathsf{v}_i \in \mathsf{W}} \omega(\mathsf{v}_i) \geq \Omega$. Let $W = \{v_i \mid \mathsf{v}_i \in \mathsf{W}\}$ be the set of regular precinct nodes corresponding to the vertices in $\mathsf{W}$. Then we have $\abs{W} = M$ and thus $\rho(W) = 2M^2 \Omega$. Furthermore, we have
\begin{align*}
    \sum_{v \in W \cap B_\Pi} \gamma(v) \tau(v) = \sum_{v \in W} \gamma(v) \rho(v) &= \sum_{i: \mathsf{v}_i \in \mathsf{W}} \Paren{\Paren{\frac{M-1}{2M}+\frac{\omega(\mathsf{v}_i)}{2\Omega}} \cdot 2M \Omega}\\
    &\geq \Paren{\frac{M-1}{2} + \frac{\Omega}{2\Omega}} \cdot 2M \Omega = M^2 \Omega = c \cdot \tau(W).
\end{align*}
Since $W$ induces a connected subgraph of $G$, it is a red $c$-deviating group of $\Pi$.

For the other direction, suppose the \audit\ instance is a $\texttt{Yes}$ instance, i.e., there is a red $c$-deviating group $W$ of $\Pi$. Suppose $W$ contains at least one auxiliary precinct node $u_i$. Recall that $\rho(W) = 2M^2 \Omega$. Hence, we have 
\[ \sum_{v \in W \cap B_\Pi} \gamma(v) \tau(v) = \sum_{v \in W} \gamma(v) \rho(v) < \sum_{v \in W \setminus \{u_i\}} \rho(v) = 2M \Omega \leq M^2 \Omega = c \cdot \tau(W), \]
a contradiction. Hence $W$ can only contain regular precinct nodes.
Then we have $\abs{\mathsf{W}} = M$, and
\begin{align*}
    \sum_{\mathsf{v}_i \in \mathsf{W}} \omega(\mathsf{v}_i) &= \sum_{v \in W \cap B_\Pi} \Paren{2\Omega \gamma(v) -\frac{(M-1)\Omega}{M}}\\
    &= \frac{1}{M} \cdot \sum_{v \in W} \Paren{\gamma(v) \rho(v) - (M-1)\Omega}\\
    &\geq \frac{\rho(W)}{M} - (M-1) \Omega = M \Omega - (M-1) \Omega = \Omega.
\end{align*}
Since $\mathsf{W}$ induces a connected subgraph of $\mathsf{G}$, the corresponding \ckspb\ instance is a $\texttt{Yes}$ instance.

Combining the above, there is a polynomial-time reduction from \ckspb\ to \audit. Since \audit\ is trivially in \textsf{NP}, we conclude that it is \textsf{NP}-complete.
\end{proof}

We then observe that the same reduction also gives the hardness of \generation.
\begin{theorem} \label{thm:gen_hardness}
\generation\ is \textsf{NP}-complete.
\end{theorem}
\begin{proof}
Observe that in each \audit\ instance constructed in the proof for Theorem~\ref{thm:audit_hardness}, the associated plan $\Pi$ is the only feasible redistricting plan. To see this, notice that every auxiliary node $u_i$ has a single neighbor $v_i$ and does not possess enough population to form a feasible district itself, and thus every $u_i$ must be paired with its corresponding $v_i$ to make a district. Therefore, the \audit\ and \generation\ are identical on this family of instances, and the hardness of \generation\ follows from the same reduction.
\end{proof}

\subparagraph{Remarks.} We note that the proofs above still hold even if we add more edges to the constructed graph. More specifically, for both the proof of Theorems~\ref{thm:audit_hardness} and~\ref{thm:gen_hardness}, we can safely add edges as long as (i) planarity is preserved and (ii) at least one of the endpoints of each additional edge is an auxiliary precinct node. To see this, observe that adding additional edges does not impact the feasibility of $\Pi$, and since valid deviating groups contain only regular precinct nodes, the set of possible deviating groups for $\Pi$ remains identical. For the proof of Theorem~\ref{thm:gen_hardness}, the additional edges may allow multiple feasible redistricting plans, but each of the feasible redistricting plans must still contain $k$ districts of one regular and one auxiliary precinct node each, and by the same reduction, either all or none of them are locally fair (corresponding to $\texttt{Yes}$ and $\texttt{No}$ \ckspb\ instances).

Note further that in both \audit\ and \generation, we do not explicitly require the districts and deviating groups to be compact with respect to any specific criteria. Under certain restrictive compactness constraints, the problems may become tractable. For example, if the districts and deviating groups are restricted to be subsets of precincts fully contained in a circle centered around a precinct point, then the set of possible districts and deviating groups has polynomial size, and thus \audit\ can be solved by enumeration in polynomial time. 

==> old/audit_results.tex <==


% Change into a histogram-- show the top maps of $2016$ are fair for the $2012$ election, use the whole ensemble as a benchmark both sets of maps perform better. 

% \begin{figure}[!htbp]
% \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/pop_dg_12.png}
%     \caption{population in deviating groups, 2012}
%     \label{fig:pop_dg_12}
%     \end{subfigure}
%     %
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/unhp_pop_dg_12.png}
%     \caption{unhappy population in deviating groups, 2012}
%     \label{fig:unhp_pop_dg_12}
%     \end{subfigure}
    
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/pop_dg_16.png}
%     \caption{population in deviating groups, 2016}
%     \label{fig:pop_dg_16}
%     \end{subfigure}
%     %
%     \begin{subfigure}[t]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/NC_2012_vs_2016/unhp_pop_dg_16.png}
%     \caption{unhappy population in deviating groups, 2016}
%     \label{fig:unhp_pop_dg_16}
%     \end{subfigure}
    
% \caption{Histograms of total (unhappy) population in deviating groups cross-compared between 2012 and 2016 North Carolina elections.}
% \end{figure}

% \begin{figure}[!htbp]
% \centering
%     \begin{subfigure}[b]{0.9\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/box_plots/NC_12_vs_16_in_12.png}
%     \caption{Performance in 2012 Election.}
%     \label{fig:nc_12_vs_16_in_12}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.9\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/box_plots/NC_12_vs_16_in_16.png}
%     \caption{Performance in 2016 Election.}
%     \label{fig:nc_12_vs_16_in_16}
%     \end{subfigure}

% \caption{Distributions of total (unhappy) population in deviating groups cross-compared between 2012 and 2016 North Carolina elections.}
% \end{figure}

==> old/dp_on_tree.tex <==
\section{Auditing for Fairness}


We detail our algorithm and the experimental results in Appendix~\ref{s:apdx_treedp}.



==> old/old-main.tex <==
% \section{Introduction}
% Let $G$ be a planar graph with vertex weights $w_v: V \rightarrow \reals^+$. 
% Let $W = \sum_{v \in V} w_v$ be the total population represented by $G$. 
% Suppose we compute a partition of the vertices. Let $k$ be the target number of districts. 

% A partition $P = P_1, \dots, P_k$ where $P_i \subseteq V$ is \emph{balanced} if for each part $P_i$: $\abs{P_i} = O(W/k)$.


% Our overall goal is to compute a balanced, compact, fair districting. 

\section{Summary of Related Work}
Census blocks are treated as indivisible in most cases, and give enough granularity to divide into balanced districts, as the number of blocks is much larger than the number of districts.
Census tracts are statistical subdivisions of a county that aim to have roughly 4,000 inhabitants. 
North Carolina has 2,195 census tracts, and 6,155 block groups.

\paragraph{Recombination Algorithm.}(Duchin et al. survey~\cite{deford2019recombination})
\begin{itemize}
    \item Recombination includes a large class of redistricting algorithms based on a large step MCMC. It works by redefining districts on a large scale in each step, rather than reassigning a small number of vertices on the boundaries between current districts (known as flip methods).  
    \item The algorithm needs some seed or initial map. During each phase chooses to merge $2$ or more districts, and then somehow randomly repartitions into approprioately sized districts. 
    \item How to repartition the merged area changes depending on the implementation, but the most common method is to find a spanning tree of the area and choosing a cut of this tree. This is shown to have good properties in~\cite{procaccia2021compact}. 
    \item Overall, the goal is not to sample uniformly from the space of all plans (most of which would be `bad'), but rather to sample from the space of compact plans. 
    \item Used to audit plans: see https://gerrymander.princeton.edu/, they compare proposed plans with average scores from an ensemble of maps generated by recomb. 
\end{itemize}

Recomb/Gerrychain is said to have the following nice properties: 
\begin{itemize}
    \item Gives a distribution over seat count, so that anomolies correspond to unfair maps.
    \item Compactness (Princeton group uses both Reock and and Polsby-Popper), also see~\cite{procaccia2021compact}
    \item Partisanship 
\end{itemize}

\begin{itemize}
    \item Edge weights correspond to geometric distance: trying to compute a Voronoi-type/power diagram on graph. The `compactness' arises from the properties of the diagram (small number of sides?). Downside may be that in dense areas (high population areas), the cost of the region will be low, so the emphasis on minimizing cost will focus on the sparse areas of the graph. See ~\cite{gawrychowski2021voronoi}. 
    \item No edge weights? This is the model used in~\cite{AKMforc2021}, where they focus on optimality. Instead, if we consider approximation there are known results (partition into $k$ balanced parts, minimizing the cut capacities, see ~\cite{andreev2006balanced}). 
    \item Edge weights related to population: correspond to willingness to cut an edge: if a vertex has small weight (low population), maybe we can cut its edges with low penalty, whereas two connected vertices of high weight should not be cut. Downside of this may be the edge weights do not make a metric.
\end{itemize}


% \paragraph{Redistricting Algorithms.}(Becker and Solomon survey~\cite{becker2020redistricting})

\section{Experiments Setup/Overview}
\begin{itemize}
    \item 1k maps generated for North Carolina, each seeded with the electoral map for the 2016 election and is the result of a 1k-step ReCom chain. Outcomes are generated with 2016 presidential election results. A $2\%$ deviation in population of a district from the ``ideal" population was allowed (corresponding to $\epsilon = 0.02$ in terms of the AAAI paper)
    \item We run the same experiment for Pennsylvania with 500 maps, each from a 10k-step Recom chain.
    \item We run the same experiment for Texas with 1k maps, each from a 10k-step Recom chain, with subsampling in auditing, that is, for auditing each map, we sample only 10k districts from the ensemble, and early-terminate if we have found 1k deviating groups.
\end{itemize}

%\newpage

\subsection{Summary of NC Results}
\begin{itemize}
    \item For NC: Out of $1,000$ maps in the ensemble, rather few ($47$ of them) are deviating group-free when audited by the set of $13,000$ districts generated. Among the other $953$ maps with deviating groups, $453$ admit $55\%$ majority deviating groups, and $210$ admit $60\%$ majority deviating groups. Thus, many maps had deviating groups that only achieved something close to a simple majority.
    \item For NC: In $46$ of the $47$ maps without deviating groups, the seat distribution is either blue 5: red 8, or blue 6: red 7. One is blue 7: red 6. Several other blue 7: red 6 plans have a few deviating groups. Plans with other kinds of seat results have many deviating groups.
\end{itemize}

\begin{figure}[!htbp]
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/DGs.png}
    \caption{North Carolina - 50\% deviating groups}
    \label{fig:nc_dgs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/55DGs.png}
    \caption{North Carolina - 55\% deviating groups}
    \label{fig:nc_55_dgs}
    \end{subfigure}

    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/DGs.png}
    \caption{Pennsylvania - 50\% deviating groups}
    \label{fig:pa_dgs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/55DGs.png}
    \caption{Pennsylvania - 55\% deviating groups}
    \label{fig:pa_55_dgs}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/DGs.png}
    \caption{Texas - 50\% deviating groups}
    \label{fig:tx_dgs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/55DGs.png}
    \caption{Texas - 55\% deviating groups}
    \label{fig:nc_55_dgs}
    \end{subfigure}
\caption{Empiricial CDF of the number of deviating group found, when we audit the maps using the districts in the ensemble. Note that we use the entire collection of districts for NC and PA, but a subsampled set for TX. \\
When the threshold for deviating groups is a simple majority, for all three states, there are relatively few fair maps w.r.t. deviating groups. When the bar is raised up to 55\%, NC and TX still have a lot of unfair maps, but almost all maps in the PA ensemble become fair.}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/DGPrecincts.png}
    \caption{North Carolina.}
    \label{fig:nc_DG_precincts}
    \end{subfigure}
    \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/DGPrecincts.png}
    \caption{Pennsylvania.}
    \label{fig:pa_DG_precincts}
    \end{subfigure}
    \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/DGPrecincts.png}
    \caption{Texas.}
    \label{fig:tx_DG_precincts}
    \end{subfigure}
    \caption{Empirical CDF of total number of precincts in deviating groups. Red precincts are the unhappy ones in the associated deviating groups (they ``initiate'' the deviation), while blue precincts are happy ones ``pulled in''. The total number of blue ones are slightly more than that of red ones, as usually a ``core'' of unhappy precincts can ``pull in'' random neighboring happy ones.}
\end{figure}


\begin{figure}[!htbp]
    \captionsetup{justification=centering}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/Seats.png}
    \caption{NC Whole ensemble \\ (AVG = 5.06, STD = 0.91)}
    \label{fig:nc_seats}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/SeatsLDG.png}
    \caption{NC Top-10\% fair maps \\ (AVG = 5.63, STD = 0.54)}
    \label{fig:nc_seats_ldg}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/SeatsHDG.png}
    \caption{NC Top-10\% unfair maps \\ (AVG = 4.51, STD = 1.29)}
    \label{fig:nc_seats_hdg}
    \end{subfigure}
    
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/Seats.png}
    \caption{PA Whole ensemble \\ (AVG = 6.87, STD = 0.73)}
    \label{fig:pa_seats}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/SeatsNDG.png}
    \caption{PA Top-14\% fair maps \\ (AVG = 7.19, STD = 0.49)}
    \label{fig:pa_seats_ldg}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/SeatsHDG.png}
    \caption{PA Top-14\% unfair maps \\ (AVG = 6.99, STD = 0.73)}
    \label{fig:pa_seats_hdg}
    \end{subfigure}
    
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/Seats.png}
    \caption{TX Whole ensemble \\ (AVG = 15.17, STD = 1.29)}
    \label{fig:tx_seats}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/SeatsLDG.png}
    \caption{TX Top-10\% fair maps \\ (AVG = 16.02, STD = 1.03)}
    \label{fig:tx_seats_ldg}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/SeatsHDG.png}
    \caption{TX Top-10\% unfair maps \\ (AVG = 14.33, STD = 1.50)}
    \label{fig:tx_seats_hdg}
    \end{subfigure}    

    \captionsetup{justification=raggedright}
    \caption{Empirical seat distribution among the generated maps: (1) whole ensemble, (2) maps whose number of precincts involved in deviating groups are near the bottom in the ensemble, i.e., ``fairest'' maps, including those without deviating groups, (3) maps whose number of precincts involved in deviating groups are near the top in the ensemble, i.e., ``most unfair'' maps. For NC and TX we use 10\% as a threshold, whereas for PA we use 14\%, as there are 14\% of them without any deviating groups. \\ 
    Somewhat intuitively, fairer maps are a bit more ``balanced'' in terms of seat distribution than the average map in the ensemble, especially for NC. For all three states, the outcome in fairer maps slightly favors blue (the minority) than in an average map; for NC and TX, the outcome in unfair maps favors red (the majority) than in an average map, but this is not the case for PA. \\
    For all three states, the fair maps have a significantly smaller variance in terms of the seat distribution than the unfair maps. (Note that the number of samples of fair and unfair maps all match, so the variances are comparable.)
    }
\end{figure}

\begin{figure}[!htbp]
    \captionsetup{justification=centering}
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/Partisanship.png}
    \caption{NC, Whole ensemble \\ (AVG = 58.73\%, STD = 1.00\%)}
    \label{fig:nc_partisanship}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/PartisanshipNDG.png}
    \caption{NC, Maps without deviating groups \\ (AVG = 59.69\%, STD = 0.93\%)}
    \label{fig:nc_partisanship_NDG}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/Partisanship.png}
    \caption{PA, Whole ensemble \\ (AVG = 62.92\%, STD = 0.47\%)}
    \label{fig:pa_partisanship}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/PartisanshipNDG.png}
    \caption{PA, Maps without deviating groups \\ (AVG = 63.09\%, STD = 0.43\%)}
    \label{fig:pa_partisanship_NDG}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/Partisanship.png}
    \caption{TX, Whole ensemble \\ (AVG = 64.22\%, STD = 0.60\%)}
    \label{fig:tx_partisanship}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/PartisanshipNDG.png}
    \caption{TX, Maps without deviating groups \\ (AVG = 64.59\%, STD = 0.57\%)}
    \label{fig:tx_partisanship_NDG}
    \end{subfigure}
    
    \captionsetup{justification=raggedright}
    \caption{The ``average partisanship'' of a map is measured as follows: for each map, there are 13/18/24 districts (for NC/PA/TX, respectively). For each district, we calculate the degree of majority of its winning color, so a district gets a score of 60\% if it has 60\% red points. Then we take the average of the 13/18/24 numbers. So this reflects how balanced/unbalanced an average district in the given map is likely to be. We plot this for (1) the entire ensemble and (2) the maps without deviating groups.
    \\
    For all three states, maps without deviating groups are slightly more partisan compared to an average map. For context, the range of average partisanship differ; this is [56.02\%, 62.47\%] for NC, [61.73\%, 64.09\%] for PA, and [61.86\%, 66.00\%] for TX. So the ``degree of freedom'' the Recom chain gets when drawing maps vary. However, the average partisanship is kind of a ``global'' type of measure, and cannot fully capture the (intrinsically local) fairness measured by deviating groups. There is a slight correlation between the average partisanship of a map and the fairness of it, as we shall see in the next set of figures.
    }
\end{figure}

\begin{figure}[!htbp]
    \captionsetup{justification=centering}
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/DGPrecinctsPartisanship.png}
    \caption{Average partisanship vs. total number of precincts in deviating groups, NC}
    \label{fig:nc_correlation1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{NCanalysis/DGPrecinctsSeats.png}
    \caption{Number of (blue) seats vs. total number of precincts in deviating groups, NC}
    \label{fig:nc_correlation2}
    \end{subfigure}
    
    \captionsetup{justification=centering}
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/DGPrecinctsPartisanship.png}
    \caption{Average partisanship vs. total number of precincts in deviating groups, PA}
    \label{fig:pa_correlation1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{PAanalysis/DGPrecinctsSeats.png}
    \caption{Number of (blue) seats vs. total number of precincts in deviating groups, PA}
    \label{fig:pa_correlation2}
    \end{subfigure}
    
    \captionsetup{justification=centering}
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/DGPrecinctsPartisanship.png}
    \caption{Average partisanship vs. total number of precincts in deviating groups, TX}
    \label{fig:tx_correlation1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{TXanalysis/DGPrecinctsSeats.png}
    \caption{Number of (blue) seats vs. total number of precincts in deviating groups, TX}
    \label{fig:tx_correlation2}
    \end{subfigure}
    
    \captionsetup{justification=raggedright}
    \caption{We finally wonder if there is correlation between the fairness measure (how many precincts are involved in deviating groups) and (1) the average partisanship; (2) the seat distribution. For all three states, results show that there is some kind of a (weak and negative) correlation for (1), with a $R^2$ value between 0.2 and 0.3. This (re-)manifests that partisan districts help reducing potential deviating groups. 
    \\
    There is little to none correlation for (2), so our fairness measure does not bias towards either the minority or the majority too much.
    }
\end{figure}

%\newpage

\subsection{Visualization of some maps}
\begin{figure}[!htbp]
\centering
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/map19.PNG}
    \caption{A map (no. 19) in the NC ensemble with 3 deviating groups found.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/map19+dev.PNG}
    \caption{A deviating group (shown in yellow) for map 19.}
    \end{subfigure}

    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/map8.PNG}
    \caption{A map with over 1000 deviating groups.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/map28.PNG}
    \caption{A map without deviating groups.}
    \end{subfigure}
\end{figure}

\newpage\newpage\newpage\newpage

\section{Future Experiments} 
\begin{itemize}
    \item Visualize the maps using the percentage of red or blue votes in the corresponding election \textcolor{blue}{Still need to figure out how to ``overlay" the deviating group on the original map.}
    \item For the maps without deviating groups in the ensemble, check the existence of deviating groups w.r.t. an ensemble of random spanning trees (next section)
    \item Weight each precinct by its population; we thought the precincts are roughly population-balanced, but they are not quite. \textcolor{red}{[SH: are we already doing this? are we currently weighting by population or the number of votes?]} \textcolor{blue}{We currently weight by the number of voters, not its population. This probably should change if we interpolate vote counts.}
    \item Repeat the existing auditing experiments for  interpolating vote counts
    \item Repeat the auditing for 2012: we want to know if the same maps are ``good" regardless of election. One way to determine this is by ranking the maps and looking at the intersection of the top $k$ $(20, 50, 100)$ maps. Then, we can try more sophisticated methods to compare the rankings.  
    \item Change the design of figures (e.g., using box graphs for figures 2-4?) so that the subfigures can be consolidated into one and show statistical significance (this can wait until new results)
\end{itemize}

District size is defined with respect to the total population (including individuals who did not cast a vote or are not eligible to vote). However, deviating groups require that we label indivduals as unhappy/happy based on their vote and election outcome. There are two approaches: 
\begin{enumerate}
    \item Define deviating groups with respect to the set of people who actually voted. If $R$ is the number of red votes and $B$ is the number of blue votes in the candidate deviating region, then checking for deviating groups is checking whether $R/(R+B)$ or $B/(R+B)$ is at least $1/2$. The upside of this definition is that the labels match exactly (if a person voted blue, they will be happy with the label blue). However, $R+B$ is not actually the population of the district (in fact it is likely much smaller), and even though other individuals might not vote we might want to assign them label. 
    \item Another approach is to give every individual a label in the district, even those who did not vote. The most straightforward way to do this is to interpolate using the actual vote counts. If there are $R$ red votes, $B$ blue votes, and $X$ is the total population, then we label a $R/(R+B)$-fraction of the population as red and a $B/(R+B)$-fraction of the population as blue, but we end up with $X$ labels. Then a deviating group needs to be a majority with respect to the total population. Since the number of people who voted varies by precinct (and population within precincts  varies), the approaches will fundamentally differ. The advantage of this second approach is that the measure of the deviating group is actually the same as that of the entire district. (This also makes it easier to do DP on trees as it avoids introducing yet another dimension of states while the DP already suffers from efficiency issues.)
\end{enumerate}

\section{Auditing}

\begin{itemize}
    \item Algorithmic question: given a map, find the strongest deviating group (the deviating group with the largest number of unhappy deviating points) subject to compactness, connectivity, and size constraint.
    \item The above problem is NP-hard even without compactness constraint, for which there are currently known approximation algorithms with constant approximation ratio, but they are not very trivial to implement and may not help much for our purpose (by relaxing the number of unhappy points by a factor of 4, we could miss a lot of deviating groups). 
    \item Current plan is to first generate/sample an ensemble of random spanning trees of the underlying precinct graph. For example, we generate 100 random spanning trees of the NC graph. This step is completely independent to any recom chain, partitions, or elections. (We have already done this) 
    \item Then, for any ``good map'' $\Pi$ that we identify in the preliminary auditing process, and for each random spanning tree $T$, we ask: is there any deviating group of $\Pi$ that is spanned by a subtree of $T$ and also satisfies the size constraint? (Connectivity is ensured by the subtree, and compactness is assumed here)
\end{itemize}

\subsection{DP Ideas/Details}

Let the underlying precinct graph be $G = (V,E)$, and $T$ be a spanning tree of $G$. For every precinct $v \in V$ let $b_v$ and $r_v$ denote its blue and red population/votes. (Assume every individual in the population is either blue or red, i.e., the data has been interpolated.)

Let $\Pi$ be the map that we would like to audit. $\Pi$ is technically a partition of $G$ mapping $V$ to $[m]$ where $m$ is the number of districts, but we do not need all that information. Without loss of generality, assume we are auditing for only blue deviating groups (i.e., a blue-majority subgraph that contain a lot unhappy blue points); then for each $v$ we only need: (i) $\text{pop}(v) = b_v + r_v$ (the population of precinct $v$) and (ii) the number of unhappy {\it blue} population in $v$:
$\text{uhp}(v) = \begin{cases}
0, & v \text{ is assigned to a blue district};\\
b_v, & \text{otherwise}.
\end{cases}$

\paragraph{Question.} Given $G$, $T$, $\text{pop}(v)$, $\text{uhp}(v)$, and parameters $\varepsilon$ and $\sigma$, \textcolor{blue}{decide whether there is a connected subtree $D \subset T$ such that $\sum_{v \in D} \text{pop}(v) \in [(1-\varepsilon)\sigma, (1+\varepsilon)\sigma]$ and $\sum_{v \in D} \text{uhp}(v) > \frac{1}{2} \cdot \sum_{v \in D} \text{pop}(v)$.}

\paragraph{DP states and recursion.}
For each $v \in V$ let $T_v$ be the subtree of $T$ rooted at $v$. For each $v \in V$ and $i \leq (1+\varepsilon)\sigma$, let $A[v,i]$ denote the maximum number of unhappy blue points in a subtree $D \subseteq T_v$ such that $v \in D$ and \textcolor{blue}{$\sum_{v \in D} \text{pop}(v) \leq i$}. (Changed)

If $v$ is a leaf we have 
\[ A[v,i] = \begin{cases}
\text{uhp}(v), &\, i \geq \text{pop}(v);\\
0, &\, \text{otherwise.}
\end{cases}\]

For non-leaf $v$, let $W = \text{children}(v) = \{w_1, \ldots, w_m\}$ denote the set of $v$'s childrens in $T$, and let $i' = i - \text{pop}(v)$. We have

\begin{align}
    A[v,i] = \text{uhp}(v) + \textcolor{red}{\max\limits_{\{i_j\}} \{ \sum_{j=1}^{m} A[w_j, i_j] \mid \sum_{j=1}^{m} i_j \leq i' \}}. \label{vertical_dp}
\end{align}

To compute the red part more efficiently, let $B[j,k]$ denote the maximum number of total unhappy points we can collect from (subtrees rooted at) $\{w_1, \ldots, w_j\}$, so the red part is just $B[m,i']$. Then we have
\[ B[1,k] = A[w_1,k] \]
and
\begin{align}
    B[j,k] = \max_{t \in [0,k]} B[j-1,k-t] + A[w_j, t]. \label{horizontal_dp}
\end{align}

{\color{blue}
\paragraph{Pruning.} We leverage that each $A[v,i]$ is non-decreasing in $i$ and each $B[j,k]$ is non-decreasing in $k$. 

Consider the computation of some $B[j,k]$. We maintain an upper bound $ub$ and a lower bound $lb$ of $B[j,k]$ along the computation; whenever $lb \geq ub$, we terminate the computation early and return $lb = ub$ as $B[j,k]$. Since values of $B[j,k]$ are computed in increasing order of $k$, initially, we let $lb = B[j,k-1]$. (We just let $lb = 0$ for $k = 0$.) 
Initially, we let $ub = B[j-1,k] + A[w_j, k]$. When the max function in Eq.~\ref{horizontal_dp} is evaluated in increasing order of $t$, we update:

\begin{itemize}
    \item $lb \gets \max \{ lb, B[j-1,k-t] + A[w_j, t] \}$ (this is just what the dp should do.)
    \item $ub \gets \min \{ ub, B[j-1,k-t] + A[w_j, k] \}.$ This is because that for any $t' > t$, we have
    \[ B[j-1,k-t'] + A[w_j, t'] \leq B[j-1,k-t] + A[w_j, k]. \]
    So $B[j-1,k-t] + A[w_j, k]$ is the maximum possible value of $B[j,k]$ if the function is maximized at any $t' > t$. If this is matched by $lb$, then the final maximized value will be exactly $lb$, and thus we can terminate the computation here at this $t$ (i.e., we prune all $t' > t$ in Eq. (\ref{horizontal_dp}).)
\end{itemize}

The same idea is applied to the computation of $A[v,i]$. If we have a lower bound $lb$ for $A[v,i]$ (Once again we can use $A[v, i-1]$ initially), then if $lb \geq ub = \text{uhp}(v) + \sum_{j=1}^{m} A[w_j, i']$, we immediately know $A[v,i] = lb$.
}

For each $v$, after computing all $A[v,i]$, we check if there is any $i \in [(1-\varepsilon)\sigma, (1+\varepsilon)\sigma]$ such that $A[v,i] > \frac{i}{2}$. If so, we have found a blue deviating group and we terminate the search.

\paragraph{Rounding.} This is likely too many states, so we round-and-scale $\text{pop}(v)$ to multiples of $P$. This will incur a small approximation to the size constraint. We do not round $\text{uhp}(v)$. 

\begin{itemize}
    \item Suppose we always round up. Then rounding too much led to a problem: the borderline (i.e., closer-to-50\% unhappy) deviating groups get overlooked, as we raise the bar (by rounding up the population) but kept the number of unhappy points precise (by not rounding up this number).
    \item For the nature of our data (at least for NC) we want to ideally use $P = 500$, but before pruning, $P = 1000$ was already too slow. After pruning, it was 2x faster, but still slow, and $P = 500$ is out of reach. (For $P = 2000$ or $P = 5000$, we get a huge speedup by pruning.) 
    \item (For context) For NC, it's roughly 3k nodes. Total population is roughly 9M, so one district has roughly 700k population. For $P = 1000$ that's roughly 700 population levels, so we get 3k * 700 = roughly 2M DP states. For each state the horizontal DP is $O(c \cdot 700)$, where in expectation $c = 1$, so that's roughly 1400M operations for auditing one map with one tree for one color. Currently this takes 10 minutes on our desktop with pruning.
    %\item \textcolor{red}{Immediate next step: we should use an iterative approach. First, we create a ``filtered ensemble'' consisting of only the maps that we did not find any deviating groups for in the naive auditing procedure. Then we see if any map in this ensemble has a deviating group when the rounding factor with $P = 5000$ with some 50 or 100 random trees. Since we have one-sided error, any such map must have a deviating group in exact, so we can discard it from the ensemble. Then, among the remaining maps, we repeat for $P = 2000$, then $P = 1000$ (we may need to deploy to the cluster for $1000$). We should not dig too hard into the inaccuracy issues, since any deviating group that is ``too hard to find'' is not robust anyways.}
    \item Instead of rounding all population values up, we randomly round either up or down to the threshold at each precinct, so that the expected population is preserved. (More specifically, say a precinct has $xP+y$ people where $y$ is the remainder. Then its population is rounded to $xP$ with probability $\frac{P-y}{P}$ and to $(x+1)P$ with probability $\frac{y}{P}$. (This created some zero-population precincts, which triggered some bugs. We fixed the algorithm so that it correctly handles such precincts with ``zero population'' and ``nonzero unhappy population''.) Again, we leave the number of unhappy points as fixed. The hope is that the total population in an aggregated district is not too far off from the actual population. 
    
    We run the DP multiple times on the same tree, since the rounding might change the result. If none deviating group is found, or some deviating group close to 50\% is found in only some of the trials, we should conclude that there is no robust deviating group of the given map w.r.t. the given tree.
    
    Empirically:
    {\color{blue}
    \begin{itemize}
        \item The DP found ``bogus deviating groups'' after the population is rounded at random. It naturally favors rounded-down precincts -- if some precinct's population is rounded down to $0$, the associated unhappy points basically ``come for free''. Often, when the DP thinks it has found a deviating group, it is under-estimating the population of the subgraph, so either the deviating group is bogus (the unhappy color is not actually a majority), or the real population is outside $[(1-\varepsilon)\sigma, (1+\varepsilon)\sigma]$ (or both). This phenomenon exists even after ``raising the bar'' -- some of the ``strong'' deviating groups (say, with the unhappy color being a $53\%$ majority) are still bogus.
        
        \item We implemented backtracking to actually recover and verify the deviating groups (so we can now save and visualize those). For each ``strong enough'' deviating groups that the DP ``found'', we audit the region again using real population numbers. If it is a bogus deviating group, we continue the DP (instead of terminating with the conclusion that the current map has a deviating group).
        
        \item Almost all deviating groups that the DP ``found'' for population range $[(1-\varepsilon)\sigma, (1+\varepsilon)\sigma]$ actually has a population over $(1+\varepsilon)\sigma$. We then modified the range to be $[(1-5\varepsilon)\sigma, (1+\varepsilon)\sigma]$. (This is to say: any ``deviating group'' with population at least $(1-5\varepsilon)\sigma$ is subject to verification.)
        
        \item For $P = 2500$, among the ``fair'' maps in the ensemble (those without deviating group in the audit-by-ensemble experiment), there exist instances in which the DP with randomized rounded population find new (verified) ``deviating groups'', sometimes for both colors. There are also maps still without deviating groups.
        
        \item We should visualize the deviating groups to see if those are indeed ``compact'' by the test of eye.
    \end{itemize}
    
    Theoretically:
    \begin{itemize}
        \item Since the said bias exists, it is not as simple as arguing that the expected real population for an arbitrary ``deviating group'' found by the algorithm is well-concentrated around the expected value.
        \item If we want to bound the error, we need to look into how the DP can exploit the rounded-down precinct nodes to build connected subtrees. 
    \end{itemize}
    }
\end{itemize}


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{fig/dp_deviating_group.png}
    \caption{A map with a red deviating group, found by the DP.}
\end{figure}



\iffalse
\begin{itemize}
    \item Algorithmic question: given a partition, find the deviating group with the largest number of unhappy deviating points. A deviating group must be compact, connected, and satisfy size constraint.
    \item Without specifying what is compact, we can relax the above problem to: given a partition, find the best connected deviating group (or report none exists) that satisfies size constraint.
    \item When the size constraint is the tightest ($\varepsilon = 0$) it reduces to the node-weighted $\sigma$-steiner tree problem, where edges are free, and $\sigma = W/k$ is the targeted size of deviating group. Given a fixed color $c$ for which we want to find deviating groups for, the node weight of a precinct node $v$ can be defined as the number of unhappy color-$c$ vertices in $v$, if we want the first objective. Note that if $v$ is color-$c$ itself then this weight is $0$.
    \begin{itemize}
        \item A $(4+\epsilon)$-approximation algorithm for planar graphs is given in~\cite{Byrka20approximating}. 
        \item The core of the algorithm is based on a primal-dual moat growing $3$-approximate algorithm for the price-collecting Steiner Tree problem, but other portions of this algorithm requires tree merging that requires extensive use of graph operations (shortest paths, etc.); without this step the solution is not connected. 
        \item If we do not want to preserve the $(4+\epsilon)$-approximate theoretical guarantee, then we can directly output the tree $T_2$ given by the core algorithm (corresponds to a good Lagrange multiplier $\lambda$ which leads to a (candidate) deviating group with slightly more than $\sigma$ population), which is likely ok in out context.
    \end{itemize}
    \item We can further relax the size constraint in the following sense: suppose the node weight of vertex $v$ is now the number of unhappy points of color-$c$ in $v$ {\it minus} the number of all other points in $v$ (including happy points of color-$c$ and points of other colors), and we just want a connected subgraph with the maximum weight (so no constraint on the size of the subgrpah). Then this is the Maximum-Node Weight Connected Subgraph (MWCS) problem.
    \begin{itemize}
        \item Several IP formulations are given in~\cite{Alvarez-Miranda13rooted} and also \url{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.727.3871&rep=rep1&type=pdf} and \url{http://www.optimization-online.org/DB_HTML/2020/08/7962.html}
        \item In~\cite{Chimani09obtaining} it is stated that formulations with polynomially-many variables/constraints does not always perform better in reality. Further, it claims that graphs with several thousands of nodes can already be solved (by IP with careful techniques) within reasonable time back in 2009. So it is maybe possible for us to directly solve this version in exact as well.
        \item Obvious drawback: maybe the best solution to this MWCS is just several ``very unhappy'' neighboring precincts, but the aggregate population is too small.
    \end{itemize}
    \item There are solvers for the MWCS problem available online: see \url{https://github.com/ctlab/virgo-solver} and \url{https://github.com/ctlab/mwcsr}. The latter seems to support a budgeted version (so we can prevent finding too large deviating groups), but this does not prevent finding too small ones.
    \item Another solver for Price-collecting Steiner Tree and MWCS: \url{https://github.com/mluipersbeck/dapcstp} (based on~\cite{Leitner18dual})
    \item Actually, if we want to utilize IP/LP for auditing and do not seek to solve some related theoretical question. Then why can't we just encode compactness using the cut size? This seems to be widely accepted.\footnote{The gerrymandering game on NYTimes -- \url{https://www.nytimes.com/interactive/2022/01/27/us/politics/congressional-gerrymandering-redistricting-game-2022.html?referringSource=articleShare} -- is likely using it. They didn't specify this explicitly, but given that the underlying graph is generic, a cut-based measure must be what they're using.} In the IP/LP the cut size comes for free as we surely have node variables. The harder question is to decide the threshold for compactness. From a data-oriented pov maybe we can use the average compactness of the existing districts in the map being audited. Or the compactness can be associated with some penalty and moved to the objective.
\end{itemize}


\section{Links/Notes}
\begin{itemize}
    \item We should do mathematical programming directly in Julia for better workflow and (possible) integration with visualization using JuMP: \url{https://github.com/jump-dev/JuMP.jl}
    \item CPLEX API for Julia: \url{https://github.com/jump-dev/CPLEX.jl}
    \item Gurobi API for Julia: \url{https://github.com/jump-dev/Gurobi.jl} \textcolor{red}{Using Gurobi 9.5 with Julia is problematic. Use 9.1.2 instead.}
\end{itemize}
\fif
